For self-supervised learning, Rationality implies generalization, provably

We prove a new upper bound on the generalization gap of classifiers that are obtained by first using self-supervision to learn a representation $r$ of the training data, and then fitting a simple (e.g., linear) classifier $g$ to the labels. Specifically, we show that (under the assumptions described below) the generalization gap of such classifiers tends to zero if $\mathsf{C}(g) \ll n$, where $\mathsf{C}(g)$ is an appropriately-defined measure of the simple classifier $g$'s complexity, and $n$ is the number of training samples. We stress that our bound is independent of the complexity of the representation $r$. We do not make any structural or conditional-independence assumptions on the representation-learning task, which can use the same training dataset that is later used for classification. Rather, we assume that the training procedure satisfies certain natural noise-robustness (adding small amount of label noise causes small degradation in performance) and rationality (getting the wrong label is not better than getting no label at all) conditions that widely hold across many standard architectures. We show that our bound is non-vacuous for many popular representation-learning based classifiers on CIFAR-10 and ImageNet, including SimCLR, AMDIM and MoCo.

==> app-theory.tex <==


\section{Simple classifiers imply small memorization gap} \label{app-theory}

In this appendix we we prove our main theoretical result (Theorem~\ref{thm:app-mainrestate}).
We will start by giving a formal definition of SSS algorithms and restating the definition of our complexity measures.

\begin{definition}[SSS Algorithms, restated] \label{def:app-SSS}
An \emph{SSS algorithm} over $(\cX\times \cY)^n$ is a procedure $T=(\Tpre,\Tfit)$ that takes as input a set $(\vx,\vy)$
and operates as follows:

\begin{enumerate}

    \item $\Tpre$ takes the (label free) data points $\vx$ as input and outputs a \emph{representation} $r:\cX \rightarrow \cR$ for some set $\cR$;
    
    \item On input the points $\{ (r(x_i),y_i) \}_{i=1}^n$, $\Tfit$ outputs a \emph{simple classifier} $g:\cR :\rightarrow \cY$;
    
    \item The output is a classifier $f:\cX \rightarrow \cY$ defined as $f(x)=g(r(x))$ for every $x\in\cX$.
\end{enumerate}
\end{definition}

We now restate the definitions of our complexity measure.



\begin{definition}[Complexity of training procedures, restated] \label{def:app-complexity}
Let $T$ be a training procedure taking as input $( \vr,\vy)= \{(r_i,y_i) \}_{i=1}^n \in (\cR \times \cY)^n$ and outputting a classifier $g:\vr\to \cY$ and  let $\eta>0$.
For every training set $(\vr,\vy)$:

\begin{itemize}
    \item The \emph{minimum description length} of $T$ with respect to $\vr,\vy,\eta$ is defined as $\cmdl_{\vr,\vy,\eta}(T)= H(g)$ where $g$ is the random variable $T(\vr,\tilde{\vy})$ in the $\eta$ noisy experiment.
    \item The \emph{prediction complexity} of $T$ with respect to $\vr,\vy,\eta$ is defined as,
$$
\ccmi_{\vr,\vy,\eta}(T) \defeq \sum_{i=1}^n I( g(r_i) ; \tilde{y}_i)
$$
where $g(r_i)$ and $\tilde{y}_i$ are viewed as random variables over the sample space induced by choosing $\tilde{\vy}$ according to the $\eta$-noisy experiment w.r.t. $\vy$ and letting $g=T(\vx,\tilde{\vy})$.

\item The \emph{deviation complexity of $T$ with respect to $\vr,\vy,\eta$}  is defined as

$$\cmi_{\vr,\vy,\eta}(T) \defeq n \cdot I(\Delta;N)$$ where $\Delta = g(r_i)-y_i \pmod{|\cY|}$ and  $N=\tilde{y}_i -{y}_i \pmod{|\cY|}$ are random variables taken over both the above sample space {\bf and the choice of $i\sim [n]$} and identifying $\cY$ with $\{0,\ldots,|\cY|-1\}$. 
\end{itemize} 
\end{definition}



The following theorem shows that $\cmi$ is upper bounded by $\ccmi$, which in turn is bounded by the operational entropy of $g$.


\begin{theorem}[Relation of complexity measures] \label{thm:app-relations}
For every $\vr,\vy,\eta>0$, and $T$
\[
 \cmi_{\vr,\vy,\eta}(T) \leq \ccmi_{\vr,\vy,\eta}(T) \leq \cmdl(T)
\]
where $g$ is the classifier output by $T$ (considered as a random variable).
\end{theorem}

\begin{proof}
Fix $T,\vr,\vy,\eta$. We get $\tilde{\vec{y}}$ by choosing i.i.d random variables $N_1,\ldots,N_n$, each equalling $0$ with probability $1-\eta$ and uniform otherwise,
and letting $\tilde{y}_i = y_i + N_i \pmod{|\cY|}$.

We start by proving the second inequality $\ccmi_{\vr,\vy,\eta}(T) \leq H(g)$.
Let $g=T(\vr,\tilde{\vec{y}})$ and define $\vec{p}=(g(r_1),\ldots,g(r_n))$ be the vector of predictions.
Then,

\begin{equation}
\ccmi_{\vr,\vy,\eta}(T) = \sum_i I(p_i; \tilde{y}_i) = \sum_i I(p_i ; N_i)
\label{eq:compbound1}
\end{equation}

with the last equality holding since for fixed $y_i$, $N_i$ determines $\tilde{y}_i$ and vice versa.
However, since the full vector $\vec{p}$ contains only more information than $p_i$, the right-hand side of (\ref{eq:compbound1}) is at most  $\sum_{i=1}^n I(\vec{p};N_i) \leq I(\vec{p}\,;\,N_1,\ldots,N_n)$, using the fact that $N_i$ random variables are independent (see Lemma~\ref{lemma2}).
For a fixed $\vr$, the value of $\vec{p}$ is completely determined by $g$ and hence the entropy of $\vec{p}$ is at most $H(g)$, establishing the second inequality of the theorem.

We now turn to the first inequality $\cmi_{\vr,\vy,\eta}(T) \leq \ccmi_{\vr,\vy,\eta}(T)$.
Let $\Delta_i = p_i - y_i \pmod{|\cY|}$.
Then,

\begin{equation}
\tfrac{1}{n}\ccmi_{\vr,\vy,\eta}(T) = \E_{j\sim [n]} I(p_j;N_j) =  \E_{j\sim [n]} I(\Delta_j;N_j)
\label{eq:compbound2}
\end{equation}

since $p_i$ determines $\Delta_i$ and vice versa.
But, since $N_j=N|i=j$  and $\Delta_j=\Delta|i=j$ (where $N,\Delta$ are the random variables defined in Definition~\ref{def:app-complexity}), the right-hand side  of (\ref{eq:compbound2}) equals

\begin{equation}
\E_{j \sim [n]} I(\Delta;N|i=j) = \E_{j\sim [n]} H(N|i=j) - H(N|\Delta,i=j)  \;.
\label{eq:compbound3}
\end{equation}
Since $N_1,\ldots,N_n$ are identically distributed, $H(N|i=j)=H(N)$ which means that the right-hand side of (\ref{eq:compbound3}) equals 
$$
H(N) - \E_{j \sim [n]} H(N|\Delta,i=j) \geq H(N) - H(N|\Delta) = I(\Delta;N) \,
$$
with the inequality holding since on average conditioning reduces entropy.
By definition $I(\Delta;N)=\tfrac{1}{n}\cmi_{\vr,\vy,\eta}(T)$, establishing what we wanted to prove.
\end{proof}


The complexity measures $\ccmi$ and $\cmi$ are defined with respect to a \emph{fixed} train set $(\vr,\vy)$, rendering them applicable for single training sets such as CIFAR-10 and ImageNet that arise in practice.
If $\cD$ is a distribution over $(\vr,\vy)$, then we define the complexity measures $\ccmi$ and $\cmi$ with respect to $\cD$ as the average of the corresponding measure with respect to $(\vr,\vy) \sim \cD$.
We now restate Theorem~\ref{thm:main}:

\begin{theorem}[Theorem~\ref{thm:main}, restated] \label{thm:app-mainrestate}
Let $T= (\Tpre,\Tfit)$ be a training procedure obtained by first training $\Tpre$ on $\vx\in \cX^n$ to obtain a representation $r:\cX \rightarrow \cR$ and then training $\Tfit$ on $(r(\vx), \vy))$ where $\vy\in \cY^n$ to obtain a classifier $g:\cR \rightarrow \cY$.
Then, for every noise parameter $\eta>0$ and distribution $\Dtrain$ over $(\cX,\cY)^n$,
$$
\text{\textcolor{memorization}{Memorization gap}}(T) = \TrainAcc_{\Dtrain,T}(\eta) - \NTrainAcc_{\Dtrain,T}(\eta) \leq \sqrt{\tfrac{\cmi_{\cR,\eta}(\Tfit)}{2n}} \cdot \frac{1}{\eta} 
$$
where $\cR$ is the distribution over $(\cR \times \cY)^n$ induced by $\Tpre$ on $\Dtrain$.
\end{theorem}

Note that the bound on the right-hand side is expressed only in terms of the complexity of the second stage $\Tfit$ and is independent of the complexity of $\Tpre$. The crux of the proof is showing (close to) independence between the corrupted indices and prediction deviation of $g$ resulting from the noise.



\begin{proof}
Let $(\vr,\vy)$ be sampled by first drawing $(\vx,\vy) \sim \Dtrain$ over $(\cX\times\cY)^n$ then applying $\vr=r(\vx)$ where $r=\Tpre(\vx)$.
Consider the sample space of sampling $\tilde{\vy}$ according to the $\eta$-noisy distribution with respect to $Y$, computing $g=\Tfit(\vr,\tilde{\vy})$,  and sampling $i \sim [n]$.
We define the following two Bernoulli random variables over this sample space:



$$Z = \characteristic_{\Delta = 0} = \begin{cases}
1 & g(R_i)=y_i\\
0 & otherwise
\end{cases}; \quad \quad B = \characteristic_{N\ne0} = \begin{cases}
1 & \tilde{y}_i \ne y_i\\
0 & otherwise
\end{cases}.$$

For a given $\vr,\vy$, since $Z$ is determined by $\Delta$ and $B$ is determined by $N$,  $I(Z;B) \leq I(\Delta; N)= \cmi_{\vr,\vy,\eta}(\Tfit)/n$.
By Lemma~\ref{lem:bernoullirv}, for every Bernoulli random variables $B,Z$

$$\left| \E[Z] - \E[Z | B=1] \right|  \leq \sqrt{\tfrac{1}{2}I(Z;B)}/ \E[B]$$

And hence in our case (since $\E[B]=\eta$),

$$\E[Z] - \E[Z|B=1] \leq \sqrt{\tfrac{\cmi_{\vr,\vy,\eta}(\Tfit)}{2n}} \cdot \tfrac{1}{\eta}\;.$$

But $\E[Z]$ corresponds to the probability that $g(r)=y$ for $(r,y)$ in the train set, while $\E[Z|B=1]$ corresponds to this probability over the noisy samples.
Hence the memorization gap is bounded  by

$$
\E_{(\vr,\vy) \sim \cR} \left[\sqrt{\tfrac{\cmi_{\vr,\vy,\eta}(\Tfit)}{2n}} \cdot \tfrac{1}{\eta} \right] \leq \tfrac{1}{\eta} \sqrt{\E_{(\vr,\vy) \sim \cR} \left[ \tfrac{\cmi_{\vr,\vy,\eta}(\Tfit)}{2n} \right]}  = 
\sqrt{\tfrac{\cmi_{\cR,\eta}(\Tfit)}{2n}} \cdot \frac{1}{\eta} 
$$
using the Jensen inequality and the concavity of square root for the first inequality.
\end{proof}

\section{Positive rationality gap leaves room for improvement} \label{sec:perfontable}

In this appendix, we prove the ``performance on the table theorem'' that states that we can always transform a robust training procedure with a positive rationality gap into a training procedure with better performance:

\begin{theorem}[Performance on the table theorem, restated] \label{thm:app-perfontable}
For every training procedure $T$ and $\Dtest,n,\eta$, if $\Dtrain =  \Dtest^n$ there exists a training procedure $S$ such that 
\begin{equation}
\TestAcc_{S,\cD,n}(\eta) \geq \NTrainAcc_{T,\cD,n}(\eta) -o(1) \label{eq:perfontable}
\end{equation} 
where $o(1)$ is a term that vanishes with $n$, and under the assumption that $\TrainAcc_{T,\cD,n}(\eta)  \geq \NTrainAcc_{T,\cD,n}(\eta)$.
\end{theorem}

For any reasonable training procedure $T$, performance on noisy train samples will not be better than the overall train accuracy, and hence the assumption will be satisfied.
In particular (since we can always add noise to our data), the above means that we can obtain a procedure $S'$ whose clean test performance is at least  $\TestAcc_T(\eta) + \Delta$ where $\Delta=\NTrainAcc_T(\eta) - \TestAcc_T(\eta)$ is the \emph{rationality gap} of $T$.
Hence if the rationality gap is larger than the robustness gap, we can use the above to improve the test performance of ``irrational'' networks.
(Note that the robustness gap of almost all standard training procedure is at most $\eta$ and in fact often much smaller.)
We stress that the procedure of Theorem~\ref{thm:perfontable}, while running in ``polynomial time'', is not particularly practical, since it makes \emph{inference} be as computationally expensive as training.
However, it is a proof of concept that irrational networks are, to some extent, ``leaving performance on the table''.

\begin{proof}
Let $T$ be a procedure as above. Our algorithm $S$ would be the following:

\begin{itemize}
    \item \textbf{Training:} The algorithm will not do any training but on input labels $D=\{ (x_i,\tilde{y}_i) \}$ simply stores these labels.
    
    \item \textbf{Inference:} On input a data point $x$, Algorithm $S$ will choose $i \in [n]$ at random, and run $T$ on the data $D$ replacing the $i$-th sample with $(x,\tilde{y})$ where $\tilde{y}$ is chosen uniformly at random. The output is $f(x)$ where $f$ is the classifier output by $T$
\end{itemize}

First note that while the number of noisy samples could change by one by replacing $(x_i,y_i)$ with $(x,\tilde{y})$, since this number is distributed according to the Binomial distribution with mean $\eta n$ and standard deviation $\sqrt{(1-\eta)\eta n} \gg 1$,
this change can affect probabilities by at most $o(1)$ additive factor.
If $\cY$ has $k$ classes, then with probability $1-1/k$ we will make $(x,\tilde{y})$ noisy ($y\ne \tilde{y}$) in which case the expected performance on it will be $\NTrainAcc_T(\eta)$. With probability $1/k$, we choose the correct label $y$ in which case performance on this sample will be equal to the expected performance on clean samples which by our assumptions is at least $\NTrainAcc_T(\eta)$ as well.
\end{proof}






==> rrm-bound.tex <==

\section{Formalization of the RRM Bound}

\begin{figure}[h]
    \centering
    \includegraphics[width=6in]{images/introplot.jpg}
    \caption{The RRM bound, as well as our analytic upper bound on it, for a variety of architectures on the ImageNet dataset. One can see that the memorization gap explains the bulk of the generalization gap, and that the RRM bound is often tight or close to tight, and that our analytic bound is often non-vacuous.  See Section~\ref{sec:experiments} for a more extensive discussion of our experiments, including a description of all the architectures considered. }
    \label{fig:introduction}
\end{figure}



We now state our results formally.
We start by introducing some notation (see also Table~\ref{tab:acc}).
Let $\cX,\cY$ be some sets and  $\cD = (\Dtrain,\Dtest)$ be a pair of distributions over $(\cX\times \cY)^n$ and $\cX\times \cY$ respectively.
(Typically $\Dtrain$ is obtained by $n$ independent copies of $\Dtest$.)
A \emph{training procedure} with respect to $\cD$ is an algorithm $T$ that takes as input $(x_i,y_i)_{i\in[n]} \sim \Dtrain$ and outputs  a classifier $f:\cX \rightarrow \cY$.
We make no assumptions on the type of classifier output, or the way that it is computed.
(The RRM bound holds for all training procedures, though it is not tight for all of them.) 
The \emph{train accuracy} of $T$, denoted by $\TrainAcc_{\cD,T}$ is the probability (over the training samples, the randomness in the procedure, and the choice of $i\in [n]$) that $f(x_i)=y_i$.
The \emph{test accuracy} of $T$, denoted by $\TestAcc_{\cD,T}$ is the probability (over training samples, randomness in procedure, and a fresh sample $(x,y) \sim \Dtest$) that $f(x)=y$.
For $\eta>0$, the \emph{$\eta$-noisy training experiment} is obtained by outputting $f= T\left( \{ (x_i,\tilde{y}_i ) \}_{i=1}^n \right)$ where we sample $\{(x_i,y_i)\} \sim \Dtrain$ and let $\tilde{y}_i=y_i$ with probability $1-\eta$ and $\tilde{y}_i$ uniform over $\cY$ otherwise.
We denote by by $\TrainAcc_{\cD,n,T}(\eta)$ the probability (over training samples, label noise, randomness in procedure, and $i\in [n]$) that $f(x_i)=y_i$ where $f$ is produced by $T$ from the $\eta$-noise experiment.
We denote by $\NTrainAcc_{\cD,n,T}(\eta)$ the same probability  $f(x_i)=y_i$ as above, but conditioned on the event that $y_i \neq \tilde{y}_i$.
Note that both accuracies are measured with respect to the \emph{original label} $y_i$ and not the perturbed label $\tilde{y}_i$ that was given to the training procedure.
We will often drop the subscripts $\cD$,$T$ when they can be inferred from the context.

\paragraph{The RRM bound.}
For $x\in\R$, let $x_+ = \max\{ x,0 \}$. The following bound immediately follows from the fact $x_+ \geq x$:

\medskip

\begin{fact}[RRM bound] \label{RRMbound} 
For every $\eta>0$, training procedure $T$ and distribution $\cD=(\Dtrain,\Dtest)$, 
\medskip
\begin{equation*}
\underbrace{\TrainAcc - \TestAcc}_{%
\let\scriptstyle\textstyle
\substack{\text{\textcolor{generalization}{Generalization}} \\  \text{\textcolor{generalization}{gap}}}} \leq
\underbrace{\Bigl[ \TrainAcc - \TrainAcc(\eta) \Bigr]_+}_{%
\let\scriptstyle\textstyle
\substack{\text{\textcolor{robustness}{Robustness}} \\ \text{\textcolor{robustness}{gap}}}}
+
\underbrace{\Bigl[ \NTrainAcc(\eta) - \TestAcc \Bigr]_+}_{%
\let\scriptstyle\textstyle
\substack{\text{\textcolor{rationality}{Rationality}} \\ \text{\textcolor{rationality}{gap}}}}
+
\underbrace{\Bigl[ \TrainAcc(\eta) - \NTrainAcc(\eta) \Bigr]_+}_{%
\let\scriptstyle\textstyle
\substack{\text{\textcolor{memorization}{Memorization}} \\  \text{\textcolor{memorization}{gap}}}}
\end{equation*}
\medskip
where the quantities above are all with respect to $T$ and $\cD$.
\end{fact}


The RRM bound holds for arbitrary distributions $\Dtrain,\Dtest$ and in particular applies to setting such as data augmentation where   $\Dtrain$ is not obtained via $n$ independent samples from $\Dtest$.\footnote{In this work we model data augmentation as transforming $\ell$ training samples into $n=t\cdot \ell$ samples by replacing each sample with $t$ augmented copies of it.} In fact, out of the three quantities on the right hand side, only the rationality gap refers to the test distribution.
The rationality gap  is more likely to be small the closer the train and test distributions are.

Our main theoretical result is the following:

\begin{theorem}[Memorization gap bound] \label{thm:main}
Let $T= (\Tpre,\Tfit)$ be an SSS training procedure obtained by first training $\Tpre$ on $\bX \in \cX^n$ to get a representation $r:\cX \rightarrow \cR$ and then training $\Tfit$ on $(r(\bX),\bY)$ for $\bY\in \cY^n$ to obtain a classifier $g:\cX \rightarrow \cY$.

Then for every $\eta>0$ and $\cD$:
$$
\text{\textcolor{memorization}{Memorization gap}}(T) = \TrainAcc_{T,\cD}(\eta) - \NTrainAcc_{T,\cD}(\eta) \leq O\left( \sqrt{\tfrac{\comp_\eta(\Tfit)}{n}} \cdot \frac{1}{\eta} \right)
$$
where $\comp_\eta(\Tfit)$ is a complexity measure of the second phase training procedure, which in particular is upper bounded by the number of bits required to describe the classifier $g$ (see Definition~\ref{def:complexity}). 
\end{theorem}






\bgroup
\def\arraystretch{1.5}

\begin{table}[bht]
\centering
    \begin{tabular}{|c|c|m{2.5in}|}
     \hline
 \multicolumn{3}{|c|}{Accuracy measures}\\
 \hline
         Quantity& Trained on& \quad \quad \quad \quad \quad \quad
         Measurement
         \\ 
\hline
    $\TestAcc\;\;\;$ & clean labels $\{ (x_i,y_i) \}_{i\in [n]}$ & $\Pr_{x,y}[f(x)=y]$ for fresh $(x,y) \sim \Dtest$.   \\
    
    \hline
    
    $\TrainAcc\;\;\;$ & clean labels $\{ (x_i,y_i) \}_{i\in [n]}$ & $\Pr_i[f(x_i)=y_i]$ for train sample $(x_i,y_i)$.  \\
 
 \hline
   $\TrainAcc(\eta) \; $ & $\eta$-noisy labels $\{ (x_i,\tilde{y}_i) \}_{i\in [n]}$ & $\Pr_i[f(x_i)=y_i]$ for train sample $(x_i,\tilde{y}_i)$ where $y_i$ \emph{original} label for $x_i$.   \\
 \hline
 
 $\NTrainAcc(\eta)$ & $\eta$-noisy labels  $\{ (x_i,\tilde{y}_i) \}_{i\in [n]}$ & $\Pr_i[f(x_i)=y_i | \tilde{y}_i \neq y_i]$ for train sample $x_i$ where $y_i$ \emph{original} label for $x_i$.    \\
 \hline
    \end{tabular}
\caption{The measurements of accuracy that appear in the RRM bound. Note that both $\TrainAcc(\eta)$ and $\NTrainAcc(\eta)$ measure accuracy with respect to the \emph{original} (``clean'') labels $\{ y_i \}_{i\in [n]}$ in the setting where the training procedure gets noisy labels $\{ \tilde{y}_i \}_{i\in [n]}$.} 
    \label{tab:acc}
    
\end{table}




We now briefly describe what is known and what we prove about the three gaps that appear on the right-hand side of the RRM bound. We provide some additional discussions in Appendix~\ref{app:examples}, including theoretical and empirical examples of algorithms which exhibit large values for each one of these gaps.

